Gravity current energetics and particle suspension

Gravity currents are a ubiquitous density driven flow occurring in both the natural environment and in industry. They include: seafloor turbidity currents, primary vectors of sediment, nutrient and pollutant transport; cold fronts; and hazardous gas spills. However, while the energetics are critical for their evolution and particle suspension, they are included in system scale models only crudely, so we cannot yet predict and explain the dynamics and run-out of such real-world flows. Herein, a novel depth-averaged framework is developed to capture the evolution of volume, concentration, momentum, and turbulent kinetic energy from direct integrals of the full governing equations. For the first time, we show the connection between the vertical profiles, the evolution of the depth-averaged flow, and the energetics. The viscous dissipation of mean-flow energy near the bed makes a leading order contribution, and an energetic approach to entrainment captures detrainment of fluid through particle settling. These observations allow a reconsideration of particle suspension, advancing over 50-years of research. We find that the new formulation can describe the full evolution of a shallow dilute current, with the accuracy depending primarily on closures for the profiles and source terms. Critically, this enables accurate and computationally efficient hazard risk analysis and earth surface modelling.

==> Sections/BackMatterJFM.tex <==
\backsection[Acknowledgements]{We thank the Energy and Environment institute, University of Hull, England, for hosting us both while we performed this research.
\\
We thank Sojiro Fukuda, for providing the compiled experimental data used to produce \cref{fig:ShapeFactors} and subsequent figures with the same data. We also thank Santiago Zúñiga and Sivaramakrishnan Balachandar for providing the simulation data used in \cref{fig:Bala_GeneralProperties,fig:Bala_Energetics,fig:Bala_Energetics_VolFree}, and likewise Paolo Orlandi for the data used in \cref{fig:ChannelDissipation_rough}. We thank Gary Parker for frank discussions on the successes and shortcomings of his 4-equation model on which this work is based. Finally, we thank Charlie Lloyd and Shahzad Sarwar for informative discussions of bed roughness.}

\backsection[Funding]{E.W.G.S. was supported by the Turbidites Research Group, University of Leeds (funded by AkerBP, CNOOC, ConocoPhillips, Harbour Energy, Murphy Oil, OMV, Oxy, and PetroChina) and by UKRI as a National Fellow in Fluid Dynamics (grant number EP/X028577/1); R.M.D was supported by the UK Natural Environment Research Council (grant number NE/S014535/1).}

\backsection[Declaration of interests]{The authors report no conflict of interest.}

\backsection[Author ORCID]{E.W.G. Skevington, \url{https://orcid.org/0000-0002-7709-9673}; R.M. Dorrell, \url{https://orcid.org/0000-0003-4257-7273}}

==> Sections/FrontMatterJFM.tex <==
\title{Gravity current energetics and particle suspension}
\shorttitle{Gravity current bulk energetics and particle suspension}

\author{Edward W.G. Skevington\aff{1}\corresp{\email{e.w.skevington@lboro.ac.uk}} \and Robert M. Dorrell\aff{1}}
\shortauthor{E.W.G. Skevington and R.M. Dorrell}
\affiliation{
	\aff{1} School of Architecture, Building and Civil Engineering, Loughborough University,\\ LE11 3TU, England
}

\maketitle

\begin{abstract}
	%\note{241/250 words}
	
	Gravity currents are a ubiquitous density driven flow occurring in both the natural environment and in industry. They include: seafloor turbidity currents, primary vectors of sediment, nutrient and pollutant transport; cold fronts; and hazardous gas spills. However, while the energetics are critical for their evolution and particle suspension, 
	they are included in system scale models only crudely,
	so we cannot yet predict and explain the dynamics and run-out of such real-world flows. Herein, a novel depth-averaged framework is developed to capture the evolution of volume, concentration, momentum, and turbulent kinetic energy 
	from direct integrals of the full governing equations. 
	For the first time, we show 
	the connection between the vertical profiles, the evolution of the depth-averaged flow, and the energetics.
	The viscous dissipation of mean-flow energy near the bed makes a leading order contribution, and an energetic approach to entrainment captures detrainment of fluid through particle settling.
	These observations allow a reconsideration of particle suspension, advancing over 50-years of research.
	We find that the new formulation can describe the full evolution of a shallow dilute current, with the accuracy depending primarily on closures for the profiles and source terms. Critically, this enables accurate and computationally efficient hazard risk analysis and earth surface modelling.
\end{abstract}

==> Templates/StandardMathsMacros.tex <==
%My macros for the math environment

\usepackage{xparse}
\makeatletter




%---BRACKETS----

%Normal brackets

\DeclarePairedDelimiter{\ppar}{\lparen}{\rparen}
\DeclarePairedDelimiter{\pang}{\langle}{\rangle}
\DeclarePairedDelimiter{\pbrc}{\lbrace}{\rbrace}
\DeclarePairedDelimiter{\pbrk}{\lbrack}{\rbrack}
\DeclarePairedDelimiter{\pgrp}{\lgroup}{\rgroup}

%Bracket-like structures

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\round}{\lfloor}{\rceil}

\DeclarePairedDelimiter{\eval@wdot}{.}{\rvert}
\NewDocumentCommand{\eval}{som}{%
	\IfBooleanTF{#1}
	{\eval@wdot*{#3}}
	{\IfNoValueTF{#2}{#3\rvert}{\eval@wdot[#2]{#3}}}%
}

\DeclarePairedDelimiterX{\setpred}[2]{\lbrace}{\rbrace}{\: #1 \: \delimsize\vert \: #2 \:}
\DeclarePairedDelimiter{\shock}{[}{]_{-}^{+}}
\DeclarePairedDelimiterX{\innerprod}[2]{\langle}{\rangle}{#1,#2}



%---OPERATORS---

\DeclareMathOperator{\sign}{sgn}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\minmod}{minmod}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\arcsinh}{arcsinh}
\DeclareMathOperator{\arccosh}{arccosh}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\arctantwo}{arctan2}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\expect}{\mathbb{E}}
\DeclareMathOperator{\variance}{\mathbb{V}\!ar}
\DeclareMathOperator{\covariance}{\mathbb{C}ov}
\DeclareMathOperator{\prob}{\mathbb{P}}



%---DIMENSIONLESS CONSTANTS---
%Define carefully, some of these are defined in the JFM template

%\Rey Reynolds number 
\ifdefined\Rey\else
\newcommand\Rey{\mbox{\textit{Re}}}
\fi

%\Pran Prandtl number
\ifdefined\Pran\else
\newcommand\Pran{\mbox{\textit{Pr}}} 
\fi

%\Pen Peclet number
\ifdefined\Pen\else
\newcommand\Pen{\mbox{\textit{Pe}}}
\fi

%\Fro Froude number
\ifdefined\Fro\else
\newcommand\Fro{\mbox{\textit{Fr}}}
\fi

%\Ric Richardson number
\ifdefined\Ric\else
\newcommand\Ric{\mbox{\textit{Ri}}}
\fi

%\Sch Schmidt number
\ifdefined\Sch\else
\newcommand\Sch{\mbox{\textit{Sc}}}
\fi



%---REYNOLDS AND SPATIAL AVERAGES---

%Reynolds average
\newcommand{\reavg}[1]{
	{\:\!\overline{\vphantom{\reflc{\phi}}#1}\:\!}
}
%Reynolds fluctuation
\newcommand{\reflc}[1]{
	\vphantom{\phi}#1'
}
%Spatial average
\newcommand{\spavg}[3]{%\spavgp{text}{subscript}{superscript}
	\mathrlap{\left\langle #1 \right\rangle}
	\mathrlap{\left. \phantom{\left\langle #1 \right.} \! \right._{#2}^{#3}}
	\mathmakebox[\maxof
	{\widthof{$\displaystyle \left\langle #1 \right\rangle$}}
	{\widthof{$\displaystyle \left. \phantom{\left\langle #1 \right.} \! \right._{#2}^{#3}$}}
	]{}
}
%Spatial average of Reynolds average
\newcommand{\sravg}[3]{
	\spavg{\reavg{#1}}{#2}{#3}
}



%---VECTOR---
\newcommand*\vecb[1]{\bm{#1}}
\newcommand*\vecbu[1]{\hat{\vecb{#1}}}
\newcommand*\dotp{\mathpalette\omitdummy@{0.5}}
\newcommand*\ddotp{\bm{:}}




%---CALCULUS---
%Uses the calculus syntax from the Physics package with a few modifications
%
%For fractions p/q, following applies
%\frac{p}{q}, standard
%\frac*{p}{q}, flat
%\frac**{p}{q}, flat, autosize slash
%\frac*[\size]{p}{q}, flat, slash size of \size
%
%For differential d syntax is
%\dd*[power]{measure}
%Star removes spacing
%
%For derivative df/dx, stars the same as for \frac, optional argument the order of the derivative
%\dv(frac syntax here)[order]{f}{x}
%If wanting to use a flat derivative without sizing with order, then \dv*[][n]{f}{x}
%
%For partial derivative df/dx, use \pdv with syntax as for \dv
%For mixed partial derivative d2f/dxdy, use \pdvt three arguments for f,x,y
%NOT IMPLEMENTED YET Alternatively, for d^n f/dx_1 ... dx_n use
%\pdvm(frac syntax here){n}{f}{x_1}...{x_n}

%\frac
\let\frac@nostar\frac
\DeclarePairedDelimiterX{\frac@starwdot}[2]{.}{.}{#1 \delimsize/ #2}
\NewDocumentCommand{\frac@star}{somm}{%
	\IfBooleanTF{#1}
	{\frac@starwdot*{#3}{#4}}
	{\IfNoValueTF{#2}{#3/#4}{\frac@starwdot[#2]{#3}{#4}}}%
}
\renewcommand*\frac{\@ifstar{\frac@star}{\frac@nostar}}

%\dd
\NewDocumentCommand{\dd}{som}{%
	\IfBooleanF{#1}{\,}%
	\IfNoValueTF{#2}{%Check whether optional argument is given
		\mathrm{d} #3%
	}{%
		\mathrm{d}^{#2} #3%
	}%
	\IfBooleanF{#1}{\,}%
}

%\dv
\NewDocumentCommand\dv@nostar{O{}mm}{%
	\frac@nostar{\mathrm{d}^{#1} #2}{{\mathrm{d} #3}^{#1}}
}
\NewDocumentCommand{\dv@star}{sO{}O{}mm}{%
	\IfBooleanTF{#1}{%
		\frac**{\mathrm{d}^{#2} #4}{{\mathrm{d} #5}^{#2}}%
	}{%
		\if \relax\detokenize{#2}\relax
		\frac*{\mathrm{d}^{#3} #4}{{\mathrm{d} #5}^{#3}}%
		\else
		\frac*[#2]{\mathrm{d}^{#3} #4}{{\mathrm{d} #5}^{#3}}%
		\fi
	}%
}
\newcommand*\dv{\@ifstar{\dv@star}{\dv@nostar}}

%\pdv
\NewDocumentCommand\pdv@nostar{O{}mm}{%
	\frac@nostar{\partial^{#1} #2}{{\partial #3}^{#1}}
}
\NewDocumentCommand{\pdv@star}{sO{}O{}mm}{%
	\IfBooleanTF{#1}{%
		\frac**{\partial^{#2} #4}{{\partial #5}^{#2}}%
	}{%
		\if \relax\detokenize{#2}\relax
		\frac*{\partial^{#3} #4}{{\partial #5}^{#3}}%
		\else
		\frac*[#2]{\partial^{#3} #4}{{\partial #5}^{#3}}%
		\fi
	}%
}
\newcommand*\pdv{\@ifstar{\pdv@star}{\pdv@nostar}}

%\pdvt
\NewDocumentCommand\pdvt@nostar{mmm}{%
	\frac@nostar{\partial^2 #1}{\partial #2 \partial #3}
}
\NewDocumentCommand{\pdvt@star}{sO{}mmm}{%
	\IfBooleanTF{#1}{%
		\frac**{\partial^2 #3}{\partial #4 \partial #5}%
	}{%
		\if \relax\detokenize{#2}\relax
		\frac*{\partial^2 #3}{\partial #4 \partial #5}%
		\else
		\frac*[#2]{\partial^2 #3}{\partial #4 \partial #5}%
		\fi
	}%
}
\newcommand*\pdvt{\@ifstar{\pdvt@star}{\pdvt@nostar}}



%%\pdvm
%\NewDocumentCommand\pdvm@nostar@two{mmmm}{%
	%	\frac{\partial^2 #2}{\partial #3 \partial #4}
	%}
%\NewDocumentCommand{\pdvm@star@two}{sO{}mmm}{%
	%	|#1,#2,#3,#4,#5|
	%%	\IfBooleanTF{#2}{%
		%%		\frac**{\partial^2 #4}{\partial #5 \partial #6}%
		%%	}{%
		%%		\if \relax\detokenize{#3}\relax
		%%			\frac*{\partial^2 #4}{\partial #5 \partial #6}%
		%%		\else
		%%			\frac*[#3]{\partial^2 #4}{\partial #5 \partial #6}%
		%%		\fi
		%%	}%
	%}
%\newcommand*\pdvm@nostar[1]{%
	%	\ifnum #1=2
	%		\pdvm@nostar@two%
	%	\fi%
	%}
%\newcommand*\pdvm@STAR[1]{%
	%	\ifnum #1=2
	%		\pdvm@nostar@two%
	%	\fi%
	%}
%\newcommand*\pdvm{\@ifstar{\pdvm@star}{\pdvm@nostar}}

%\def\pdvm@str@frac{frac}
%\def\pdvm@str@flat{flat}
%\def\pdvm@str@slsh{slsh}
%
%\NewDocumentCommand{\pdvm@two}{mmmmm}{
	%	F|#1,#2,#3,#4,#5|
	%}
%
%\newcommand*\pdvm@nostar[1]{%
	%	A|#1| \:
	%	\ifnum #1=2
	%		\pdvm@two{\pdvm@str@frac}{}%
	%	\fi%
	%}
%\newcommand*\pdvm@star[2]{%
	%	B%\abs{ #1 , #2 } \:
	%%	\ifnum #2=2
	%%		\pdvm@two{\pdvm@str@slsh}{#1}%
	%%	\fi%
	%}
%\newcommand*\pdvm@sstar[1]{%
	%	C|#1| \:
	%	\ifnum #1=2
	%		\pdvm@two{\pdvm@str@flat}{}%
	%	\fi%
	%}
%
%\newcommand\pdvm@staropt[1][]{%
	%	a| #1 | \:%
	%	\if \relax\detokenize{#1}\relax
	%		b%
	%		\pdvm@star{}%
	%	\else
	%		c%
	%		\pdvm@star{#1}%
	%	\fi
	%}
%\newcommand*\pdvm@STAR{\@ifstar{\pdvm@sstar}{\pdvm@staropt}}
%\newcommand*\pdvm{\@ifstar{\pdvm@STAR}{\pdvm@nostar}}



%---VECTOR CALCULUS---
%Uses similar syntax to the physics package.
%
%\grad{f}	Gradient operator
%\div{f}	Divergence operator
%\curl{f}	Curl operator

\let\divisionsymbol\div

\newcommand\grad[1]{\nabla #1}
\renewcommand\div[1]{\nabla \dotp #1}
\newcommand\curl[1]{\nabla \times #1}





%---ORDER NOTATION---

%If order is used with an empty argument then dont use parenthesis
\newcommand{\order@text}[1]{	
	\if\relax\detokenize{#1}\relax% #1 is empty
	\else% #1 is nonempty
	\ppar*{#1}%\qty(#1)
	\fi
}

%Big O
\newcommand{\order}[1]{
	\mathcal{O}\order@text{#1}
}

%Little O
\newcommand{\lorder}[1]{
	\mathchoice
	{{\scriptstyle\mathcal{O}}\order@text{#1}}% \displaystyle
	{{\scriptstyle\mathcal{O}}\order@text{#1}}% \textstyle
	{{\scriptscriptstyle\mathcal{O}}\order@text{#1}}% \scriptstyle
	{\scalebox{.6}{${\scriptscriptstyle\mathcal{O}}\order@text{#1}$}}%\scriptscriptstyle
}

%Big Theta
\newcommand{\Torder}[1]{
	\mathit{\Theta}\order@text{#1}
}




%---ASSORTED---

%%Upright math text
%\DeclareMathAlphabet{\mathup}{OT1}{\familydefault}{m}{n}

%Have equation span full width of collumn (good for equations in lists)
\newcommand{\eqnwide}{\displayindent0pt \displaywidth\textwidth}

%Use as 10^\nth
\newcommand{\nth}{\text{th}}

%Defined to be equal to
\@ifundefined{eqdef}{\newcommand{\eqdef}{\vcentcolon =}}{}%{\stackrel{\mathrm{def}}{=}}

%Text style fraction
\newcommand{\textfrac}[2] {{\textstyle\frac{#1}{#2}}}

%Omitted dummy variable as a dot
\newcommand*\omitdummy{\mathchoice
	{\omitdummy@{\displaystyle}{0.6}}
	{\omitdummy@{\textstyle}{0.6}}
	{\omitdummy@{\scriptstyle}{0.7}}
	{\omitdummy@{\scriptscriptstyle}{0.8}}
}
\newcommand*\omitdummy@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}

%Degree symbol
\newcommand{\degree}{^{\circ}}



%---ENVIRONMENTS---

%Like cases but with as many collumns as you like

\newenvironment{multicasesnobrac}[1][1]{%
	%No braces
	%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\begin{array}{*{#1}{r@{}l}}
	}{
	\end{array}
}
\newenvironment{multicases}[1][1]{%
	%Left braced
	%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\left\{\begin{array}{*{#1}{r@{}l}}
	}{
	\end{array}\right.
}
\newenvironment{multicasesd}[1][1]{%
	%Left braced with display style
	%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\left\{\begin{array}{*{#1}{>{\displaystyle}{r}@{}>{\displaystyle}{l}}}
	}{
	\end{array}\right.
}
\NewDocumentEnvironment{multlinedrel}{ O{b} O{0.9} +b }{%
	%A verseion of multlined where the default alignment of the label is bottom,
	%and the width of environment is specified relative to display width:
	%Optional arguments:
	%#1 	the alignment of the label, default b
	%#2		the relative width of the envirnoment, default 0.9
	\begin{multlined}[#1][#2\displaywidth]
		#3
	\end{multlined}%
}{}




%---SIDE BY SIDE SUBEQUATIONS---

%Multiple labeled equations on same line
\newlength{\sbsse@Wl}	%Width of left equation
\newlength{\sbsse@Wm}	%Width of mid text
\newlength{\sbsse@Wr}	%Width of right equation
\newlength{\sbsse@Wt}	%Width of tag
\newlength{\sbsse@We}	%Remaining width on line
\newlength{\sbsse@Wd}	%Remaining width divided into pieces

%Two equations side by side
\newcommand\sidebysidesubequations[6]{%
	% #1    reference label
	% #2    left subequation
	% #3    left label
	% #4    midtext
	% #5    right subequation
	% #6    right label
	
	%Setup the equations to be typed
	\def\sbsse@El{#2}
	\def\sbsse@Em{\text{#4}}
	\def\sbsse@Er{#5}
	\def\sbsse@Et{(\ref*{#1}a,b)}
	%Compute the widths
	\settowidth{\sbsse@Wl}{\begin{math}\displaystyle\sbsse@El\end{math}}
	\settowidth{\sbsse@Wm}{\begin{math}\displaystyle\sbsse@Em\end{math}}
	\settowidth{\sbsse@Wr}{\begin{math}\displaystyle\sbsse@Er\end{math}}
	\settowidth{\sbsse@Wt}{\sbsse@Et}
	\setlength{\sbsse@We}{\linewidth-\sbsse@Wl-\sbsse@Wm-\sbsse@Wr-\sbsse@Wt}
	
	%Begin equation typesetting, with label for overall subequations
	\begin{subequations}\ltx@label{{#1}}
		\begin{displaymath}
			%Left equation and label
			\sbsse@El\refstepcounter{equation}\ltx@label{{#3}}
			%Space, and midtext if any
			\if\relax\detokenize{#4}\relax
			\setlength{\sbsse@Wd}{\sbsse@We/3}
			\hspace{\sbsse@Wd}
			\else
			\setlength{\sbsse@Wd}{\sbsse@We/4}
			\hspace{\sbsse@Wd}\sbsse@Em\hspace{\sbsse@Wd}
			\fi
			%Right equation and label
			\sbsse@Er\refstepcounter{equation}\ltx@label{{#6}}
			%Tag
			\tag*{\sbsse@Et}
		\end{displaymath}
	\end{subequations}
}

%Three equations side by side
\newcommand\sidebysidesubequationsT[7]{%
	% #1    reference label
	% #2    left subequation
	% #3    left label
	% #4    mid subequation
	% #5	mid label
	% #6    right subequation
	% #7    right label
	
	%Setup the equations to be typed
	\def\sbsse@El{#2}
	\def\sbsse@Em{#4}
	\def\sbsse@Er{#6}
	\def\sbsse@Et{(\ref*{#1}a,b,c)}
	%Compute the widths
	\settowidth{\sbsse@Wl}{\begin{math}\displaystyle\sbsse@El\end{math}}
	\settowidth{\sbsse@Wm}{\begin{math}\displaystyle\sbsse@Em\end{math}}
	\settowidth{\sbsse@Wr}{\begin{math}\displaystyle\sbsse@Er\end{math}}
	\settowidth{\sbsse@Wt}{\sbsse@Et}
	\setlength{\sbsse@We}{\linewidth-\sbsse@Wl-\sbsse@Wm-\sbsse@Wr-\sbsse@Wt}
	\setlength{\sbsse@Wd}{\sbsse@We/4}
	
	%Begin equation typesetting, with label for overall subequations
	\begin{subequations}\ltx@label{{#1}}
		\begin{displaymath}
			%Left equation and label
			\sbsse@El\refstepcounter{equation}\ltx@label{{#3}}
			%Space
			\hspace{\sbsse@Wd}
			%Mid equation and label
			\sbsse@Em\refstepcounter{equation}\ltx@label{{#5}}
			%Space
			\hspace{\sbsse@Wd}
			%Right equation and label
			\sbsse@Er\refstepcounter{equation}\ltx@label{{#7}}
			%Tag
			\tag*{\sbsse@Et}
		\end{displaymath}
	\end{subequations}
}




\makeatother
